Blind Channel Estimation and Data Detection with Unknown Modulation and Coding Scheme

This paper investigates a complete blind receiver approach in an unknown multipath fading channel, which has multiple tasks including blind channel estimation, noise power estimation, modulation classification, channel coding recognition, and data detection. Each of these tasks has been sufficiently studied in the literature. However, to the best of our knowledge, this overall problem has not been investigated previously. This paper is the first attempt to address this overall problem jointly. We propose a complete blind receiver approach that jointly estimates the unknown channel state information and noise power, recognizes the unknown modulation and coding scheme, detects the data of interest, and thus named BERD receiver. Another merit of the proposed BERD receiver is that it can be implemented for both a single receiver and multiple receivers, which ensures successful estimation, recognition, and detection for such an extremely difficult problem. In addition, numerical results show the performance of the proposed receiver in three folds: a) the BERD receiver outperforms the linear minimum mean squared error (LMMSE) pilot-based channel estimator by over 3.5 dB at the MSE of 0.01; b) the correct modulation/coding recognition performance of the BERD receiver is within 0.3 dB as close to the recognition benchmark when the perfect channel state information (CSI) is available; c) the BERD receiver is within 0.5 dB at the bit error rate of 0.001 compared to the benchmark when the modulation, the channel coding, and the CSI are perfectly known. Finally, the BERD receiver finds many applications in both civilian and military scenarios, such as the interference cancelation in spectrum sharing, real-time signal interception, and processing in electronic warfare operations, automatic recognition of a detect signal in software-defined radio.

==> pream_bm.tex <==
%Environments
\newtheorem{prop}{Proposition}
\renewcommand{\theprop}{\arabic{section}.\arabic{prop}}
\newtheorem{cor}{Corollary}
\renewcommand{\thecor}{\arabic{section}.\arabic{cor}}
\newtheorem{lm}{Lemma}
\renewcommand{\thelm}{\arabic{section}.\arabic{lm}}
\newtheorem{thm}{Theorem}
\renewcommand{\thethm}{\arabic{section}.\arabic{thm}}

\newcommand{\td}{\tilde}
\newcommand{\bal}{\begin{align}}
\newcommand{\eal}{\end{align}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\benn}{\begin{eqnarray*}}
\newcommand{\eenn}{\end{eqnarray*}}
\def\IR{\rm I \kern-0.20em R}
\newcommand{\utwi}[1]{\mbox{\boldmath $ #1$}}

\newcommand{\bthm}{\begin{thm}}
\newcommand{\ethm}{\end{thm}}

\newcommand{\bcor}{\begin{cor}}
\newcommand{\ecor}{\end{cor}}
\newcommand{\bprop}{\begin{prop}}
\newcommand{\eprop}{\end{prop}}
\newcommand{\blm}{\begin{lm}}
\newcommand{\elm}{\end{lm}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ber}{\begin{eqnarray}}
\newcommand{\eer}{\end{eqnarray}}
\newcommand{\bseq}{\begin{subequations}}
\newcommand{\eseq}{\end{subequations}}


\newcommand{\opt}{^{\rm op}}


\newcommand{\balp}{\boldsymbol{\alpha}}
\newcommand{\bbt}{\boldsymbol{\beta}}

\renewcommand{\r}{\rho}

%\newenvironment{proof}{\begin{trivlist}\item[]{\bf
%Proof:\hspace{2mm}}}{\hfill$\blackbox$\end{trivlist}}
\newcommand{\bproof}{\begin{proof}}
\newcommand{\eproof}{\end{proof}}

\renewcommand{\i}{\imath}
\renewcommand{\j}{\jmath}
\newcommand{\bim}{\boldsymbol \imath}

\renewcommand{\sp}{\rm span}
\newcommand{\nul}{\rm null}
\newcommand{\calA}{\mathcal A}
\newcommand{\calB}{\mathcal B}
\newcommand{\calC}{\mathcal C}
\newcommand{\calR}{\mathcal R}
\newcommand{\calS}{\mathcal S}
\newcommand{\calK}{\mathcal K}
\newcommand{\calW}{\mathcal W}
\newcommand{\calE}{\mathcal E}
\newcommand{\calU}{\mathcal U}
\newcommand{\calV}{\mathcal V}
\newcommand{\calJ}{\mathcal J}

%Math symbol shorforms
\renewcommand{\th}{\theta}
\newcommand{\thh}{\hat{\th}}
\newcommand{\thb}{\bar{\th}}
\newcommand{\tht}{\tilde{\th}}
\newcommand{\pl}{\partial}
\newcommand{\epb}{\bar{\ep}}
\newcommand{\limsupb}{\overline{\lim}}
\newcommand{\liminfb}{\underline{\lim}}
\newcommand{\eh}{\hat{\ep}}
\newcommand{\etl}{\tilde{\ep}}
\newcommand{\gm}{\gamma}
\newcommand{\Gm}{\Gamma}
\newcommand{\sm}{\sigma}
\newcommand{\Sm}{\mathit \Sigma}
\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\bth}{\hat{\bt}}
\newcommand{\btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\tauh}{\hat{\tau}}
\newcommand{\pitl}{\tilde{\pi}}
\newcommand{\phib}{\bar{\phi}}
\newcommand{\sa}{\mathcal{F}}
\newcommand{\sah}{\hat{\sa}}
\newcommand{\satl}{\tilde{\sa}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Gch}{\hat\mathcal{G}}
\newcommand{\Gctl}{\tilde\mathcal{G}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{{\mathcal{C}}}
\newcommand{\Hc}{{\mathcal{H}}}
\newcommand{\Dsc}{{\cal D}}
\newcommand{\Ic}{{{\cal I}}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Rc}{\Re}
\newcommand{\Oc}{\mathcal{O}}
%\newcommand{\oc}{\mathcal{o}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\ah}{\hat{a}}
\newcommand{\Ahat}{\hat{A}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\ab}{\bar{a}}
\newcommand{\atl}{\tilde{a}}
\newcommand{\btl}{\tilde{b}}
\newcommand{\ctl}{\tilde{c}}
\newcommand{\hh}{\hat{h}}
\newcommand{\htl}{\tilde{h}}
\newcommand{\hb}{\bar{h}}
\newcommand{\gh}{\hat{g}}
\newcommand{\gb}{\bar{g}}
\newcommand{\fh}{\hat{f}}
\newcommand{\sh}{\hat{s}}
\newcommand{\lmh}{\hat{\lm}}
\newcommand{\xb}{\bar{x}}
\newcommand{\Jh}{\hat{J}}
\newcommand{\bhh}{\hat{\boldsymbol{h}}}
\newcommand{\bHh}{\hat{\boldsymbol{H}}}
\newcommand{\bAh}{\hat{\boldsymbol{A}}}
\newcommand{\bGh}{\hat{\boldsymbol{G}}}
\newcommand{\bgh}{\hat{\boldsymbol{g}}}
\newcommand{\bQh}{\hat{\boldsymbol{Q}}}
\newcommand{\Lambdah}{\hat{{\Lambda}}}
\newcommand{\bUh}{\hat{\boldsymbol{U}}}

%\newcommand{\bPsih}{\hat{\boldsymbol{\Psi}}}
\newcommand{\thmax}{\th_{\mbox{\scriptsize max}}}
\newcommand{\thmin}{\th_{\mbox{\scriptsize min}}}
\newcommand{\smmax}{\sm_{\mbox{\scriptsize max}}}
\newcommand{\smpmax}{\sm'_{\mbox{\scriptsize max}}}
\newcommand{\Mmax}{M_{\mbox{\scriptsize max}}}
\newcommand{\Fmax}{F_{\mbox{\scriptsize max}}}
\newcommand{\Ymax}{Y_{\mbox{\scriptsize max}}}
\newcommand{\Ypmax}{Y'_{\mbox{\scriptsize max}}}
\newcommand{\Thmax}{\Theta_{\mbox{\scriptsize max}}}
\newcommand{\Nmax}{N_{\mbox{\scriptsize max}}}
\newcommand{\Nmin}{N_{\mbox{\scriptsize min}}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Nh}{\hat{N}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ab}{\bar{A}}
\newcommand{\Au}{\underline{A}}
\newcommand{\Ru}{\underline{R}}
\newcommand{\ru}{\underline{\gamma}}
\newcommand{\AB}{\mbox{\boldmath $A$}}
\newcommand{\Bb}{\bar{B}}
\newcommand{\Bu}{\underline{B}}
\newcommand{\XB}{\mbox{\boldmath $X$}}
\newcommand{\sbx}{\mbox{\boldmath $ \scriptstyle{X} $}}
%\newcommand{\sby}{\scriptstyle{\mathbf{Y}}}
\newcommand{\sbz}{\mbox{\boldmath $ \scriptstyle{Z} $}}
\newcommand{\ZB}{\mbox{\boldmath $Z$}}
\newcommand{\XBb}{\bar{\XB}}
\newcommand{\Yb}{\bar{Y}}
\newcommand{\Rb}{\bar{R}}
\renewcommand{\DJ}{\nabla\! J}
\newcommand{\DT}{\nabla T}
\newcommand{\Dlt}{\nabla t}
\newcommand{\DC}{\nabla C}
\newcommand{\Dct}{\tilde{\Dc}}
\newcommand{\Dth}{\Delta\th}
\newcommand{\duh}{\partial}
%

%Math operators, and such
\newcommand{\cl}[1]{\overline{#1}}
\newcommand{\ir}[1]{\stackrel{\circ}{#1}}
\newcommand{\ip}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\argsup}{\mathop{\mbox{\rm arg\,sup}}}
\newcommand{\argmin}{\mathop{\mbox{\rm arg\,min}}}
\newcommand{\argmax}{\mathop{\mbox{\rm arg\,max}}}
\newcommand{\arginf}{\mathop{\mbox{\rm arg\,inf}}}
\newcommand{\rank}{\mathop{\mbox{\rm rank}}}
\newcommand{\Span}{\mathop{\mbox{\rm span}}}
\newcommand{\diag}{\mathop{\mbox{\rm diag}}}
\newcommand{\dist}{\mathop{\mbox{\rm dist}}}
\newcommand{\var}{\mathop{\mbox{\rm var}}}
\newcommand{\cov}{\mathop{\mbox{\rm cov}}}
\newcommand{\tr}{\mathop{\mbox{\rm tr}}}
\newcommand{\sgn}{\mathop{\mbox{\rm sgn}}}
\newcommand{\eqdfn}{\stackrel{\scriptscriptstyle\triangle}{=}}
\newcommand{\eqas}{\stackrel{\scriptstyle a.s.}{=}}
\newcommand{\gt}{\rightarrow}
\newcommand{\impl}{\Rightarrow}
\newcommand{\iaof}{\Leftrightarrow}
\newcommand{\blackbox}{\vrule height7pt width5pt depth1pt}

%Environments
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bdesc}{\begin{description}}
\newcommand{\edesc}{\end{description}}
\newcommand{\beqarrn}{\begin{eqnarray*}}
\newcommand{\eeqarrn}{\end{eqnarray*}}
\newcommand{\bproofof}{\begin{proofof}}
\newcommand{\eproofof}{\end{proofof}}
\newenvironment{rem}{\begin{trivlist}\item[]{\bf
Remark:}\hspace{4mm}}{\end{trivlist}}
\newcommand{\brem}{\begin{rem}}
\newcommand{\erem}{\end{rem}}
\newenvironment{rems}{\begin{trivlist}\item[]{\bf
Remarks}\begin{itemize}}{\end{itemize}\end{trivlist}}
\newcommand{\brems}{\begin{rems}}
\newcommand{\erems}{\end{rems}}
\newtheorem{fact}{Fact}
\newcommand{\bfact}{\begin{fact}}
\newcommand{\efact}{\end{fact}}
\newtheorem{examp}{Example}
\newcommand{\bexamp}{\begin{examp}\rm}
\newcommand{\eexamp}{\end{examp}}
\newtheorem{defn}{Definition}
\newcommand{\bdefn}{\begin{defn}\rm}
\newcommand{\edefn}{\end{defn}}
\renewcommand{\thedefn}{\arabic{section}.\arabic{defn}}

\newtheorem{alg}{Algorithm}
\newcommand{\balg}{\begin{alg}}
\newcommand{\ealg}{\end{alg}}

\newtheorem{prob}{Problem}
\newcommand{\bprob}{\begin{prob}}
\newcommand{\eprob}{\end{prob}}
\newcommand{\support}[1]{\renewcommand{\thefootnote}{}\footnotetext{#1}\renewcom
mand{\thefootnote}{\fnsymbol{footnote}}}
\newcommand{\twocase}[2]{\left\{\begin{array}{ll}#1 \\
#2\end{array}\right.}
\newcommand{\threecase}[3]{\left\{\begin{array}{ll}#1 \\ #2\\
#3\end{array}\right.}
\newcommand{\bvtm}{\begin{verbatim}}
\newcommand{\bfig}{\begin{figure}}
\newcommand{\efig}{\end{figure}}
\newcommand{\bfigs}{\begin{figure*}}
\newcommand{\efigs}{\end{figure*}}
\newcommand{\bcen}{\begin{center}}
\newcommand{\ecen}{\end{center}}

\def\Bbb{\mathbb }
\def\real {{\Bbb R}}
\def\nat {{\Bbb N}}
\def\cn {{\Bbb CN}}
\def\compl {{\Bbb C}}
\def\integer {{\Bbb Z}}
\def\eptn {{\Bbb E}}
\newcommand{\bIc}{{\Bbb I}}


\long\def\comment#1{}

%math operators
\newcommand{\AR}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mar}[2]{\begin{array}[t]{#1} #2 \end{array}}
\newcommand{\nn}{\nonumber \\}

%math symbol shorforms
\def\pl{(L)}
\def\sg{\sigma}
\def\Sg{\Sigma}
\def\dt{\delta}
\def\Dt{\Delta}
\def\lb{\lambda}
\def\ep{\varepsilon}
%modified on March 15, 2000
\def \scriptf{{{\cal F} }}
\def \tn{\tilde{n}}
\def \b{\beta}
\def \n2{{N_0 \over 2}}
\def \g{\gamma}
\def \G{\Gamma}
\def \et{\eta_{s1}}
\def \ett{\eta_{s2}}
%\def \bt{\bar{T}}
\def\ra{\rightarrow}
\def\lra{\longrightarrow}
\def\Lra{\Longrightarrow}
\def\st{\stackrel{a.s.}{\longrightarrow}}
\def\asst{\stackrel{a.s.}{\Longrightarrow}}
\def\pdst{\stackrel{P}{\Longrightarrow}}
\def\ard{\stackrel{(d)}{\longrightarrow}}
\def\pst{\stackrel{P}{\longrightarrow}}
\def\pist{\stackrel{\Pi}{\longrightarrow}}
\def\pitost{\stackrel{\Pi_2}{\longrightarrow}}
\def\dst{\stackrel{{\cal D}}{\Longrightarrow}}
\def\eqa{\stackrel{(a)}{=}}
\def\eqb{\stackrel{(b)}{=}}
\def\eqc{\stackrel{(c)}{=}}
\def\leqa{\stackrel{(a)}{\leq}}
\def\leqb{\stackrel{(b)}{\leq}}
\def\leqc{\stackrel{(c)}{\leq}}
\def\leqd{\stackrel{(d)}{\leq}}

%\def\Re{\mbox{\rm Re}}
%\def\Im{\mbox{\rm Im}}
\def\mmse{\mbox{\scriptsize\textrm{mmse}}}
\def\MMSE{\mbox{\textrm{MMSE}}}
\def\ms{\mbox{\scriptsize \textrm{ms}}}


\def\kK{\mbox{$k=1, \cdots, K$}}
\def\nN{\mbox{$n=1, \cdots, N$}}
\def\mM{\mbox{$m=1, \cdots, M$}}
\def\lL{\mbox{$l=1, \cdots, L$}}
\def \h5{\hspace{0.5in}}
\def \lf{ L \ra \infty}
\def \nf{ N \ra \infty}

\def \bgamma{\mbox{\boldmath $\gamma$}}
\def \bds{\mbox{\scriptsize\boldmath $d$}}


\def \bIc{\mbox{\boldmath ${\mathcal I}$}}
\def \bLambda{\mbox{\boldmath $\Lambda$}}




\def \bzr{\mbox{\boldal $0$}}
\def \bone{\mbox{\boldmath $1$}}

\newcommand{\mf}{\mbox{\scriptsize\textrm{mf}}}
\newcommand{\eff}{\mbox{\scriptsize \textrm{eff}}}
\newcommand{\SIR}{\mbox{\rm SIR}}
\newcommand{\MSIR}{\mbox{\rm MSIR}}
\newcommand{\II}{\mbox{\scriptsize{\rm II}}}
\newcommand{\SNR}{\mbox{\rm SNR}}
\newcommand{\bigo}{\mbox{\rm O}}
\newcommand{\littleo}{\mbox{\rm o}}
\newcommand{\mrc}{\mbox{\scriptsize\textrm {mrc}}}
\newcommand{\MAI}{\mbox{\scriptsize\textrm {MAI}}}
\newcommand{\egc}{\mbox{\scriptsize\textrm {egc}}}
\newcommand{\slc}{\mbox{\scriptsize\textrm {sc}}}
\newcommand{\gmdist}{\mbox{\rm Gamma}}




\newcommand{\ba}{{\boldsymbol{a}}}
\newcommand{\bb}{{\boldsymbol{b}}}
\newcommand{\bc}{{\boldsymbol{c}}}
\newcommand{\bd}{{\boldsymbol{d}}}
\newcommand{\bee}{{\boldsymbol{e}}}
\newcommand{\bff}{{\boldsymbol{f}}}
\newcommand{\bg}{{\boldsymbol{g}}}
\newcommand{\bh}{{\boldsymbol{h}}}
\newcommand{\bi}{{\boldsymbol{i}}}
\newcommand{\bj}{{\boldsymbol{j}}}
\newcommand{\bk}{{\boldsymbol{k}}}
\newcommand{\bl}{{\boldsymbol{l}}}
\newcommand{\bm}{{\boldsymbol{m}}}
\newcommand{\bn}{{\boldsymbol{n}}}
\newcommand{\bo}{{\boldsymbol{o}}}
\newcommand{\bp}{{\boldsymbol{p}}}
\newcommand{\bq}{{\boldsymbol{q}}}
\newcommand{\br}{{\boldsymbol{r}}}
\newcommand{\bs}{{\boldsymbol{s}}}
\newcommand{\bt}{{\boldsymbol{t}}}
\newcommand{\bu}{{\boldsymbol{u}}}
\newcommand{\bv}{{\boldsymbol{v}}}
\newcommand{\bw}{{\boldsymbol{w}}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\by}{{\boldsymbol{y}}}
\newcommand{\bz}{{\boldsymbol{z}}}

\newcommand{\bA}{{\boldsymbol{A}}}
\newcommand{\bB}{{\boldsymbol{B}}}
\newcommand{\bC}{{\boldsymbol{C}}}
\newcommand{\bD}{{\boldsymbol{D}}}
\newcommand{\bE}{{\boldsymbol{E}}}
\newcommand{\bF}{{\boldsymbol{F}}}
\newcommand{\bG}{{\boldsymbol{G}}}
\newcommand{\bH}{{\boldsymbol{H}}}
\newcommand{\bI}{{\boldsymbol{I}}}
\newcommand{\bJ}{{\boldsymbol{J}}}
\newcommand{\bK}{{\boldsymbol{K}}}
\newcommand{\bL}{{\boldsymbol{L}}}
\newcommand{\bM}{{\boldsymbol{M}}}
\newcommand{\bN}{{\boldsymbol{N}}}
\newcommand{\bO}{{\boldsymbol{O}}}
\newcommand{\bP}{{\boldsymbol{P}}}
\newcommand{\bQ}{{\boldsymbol{Q}}}
\newcommand{\bR}{{\boldsymbol{R}}}
\newcommand{\bS}{{\boldsymbol{S}}}
\newcommand{\bT}{{\boldsymbol{T}}}
\newcommand{\bU}{{\boldsymbol{U}}}
\newcommand{\bV}{{\boldsymbol{V}}}
\newcommand{\bW}{{\boldsymbol{W}}}
\newcommand{\bX}{{\boldsymbol{X}}}
\newcommand{\bY}{{\boldsymbol{Y}}}
\newcommand{\bZ}{{\boldsymbol{Z}}}

\newcommand{\dff}{\stackrel{\triangle}{=}}

\newcommand{\hbU}{\hat{\utwi{U}}}
\newcommand{\hbY}{\hat{\utwi{Y}}}
\newcommand{\bLam}{{\utwi{\mathnormal\Lambda}}}
\newcommand{\bPi}{{\utwi{\mathnormal\Pi}}}
\newcommand{\bPhi}{{\utwi{\mathnormal\Phi}}}
\newcommand{\bGm}{{\boldsymbol{\Gamma}}}
%\newcommand{\bSm}{\boldsymbol{\Sigma}}
\newcommand{\bDt}{\boldsymbol{\Delta}}
\newcommand{\bdt}{\boldsymbol{\delta}}
\newcommand{\bbeta}{\boldsymbol{\eta}}
\newcommand{\bep}{\boldsymbol{\ep}}

%\newcommand{\bOm}{\boldsymbol{\Omega}}
\newcommand{\bOm}{{\utwi{\mathnormal\Omega}}}
\newcommand{\bSm}{{\utwi{\mathnormal\Sigma}}}

\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bmu}{{\utwi{\mathnormal\mu}}}
\newcommand{\bPsi}{{\utwi{\mathnormal\Psi}}}
\newcommand{\bPsih}{\hat{\utwi{\mathnormal\Psi}}}

\newcommand{\bxi}{{\utwi{\mathnormal\xi}}}
\newcommand{\mDel}{ \mathnormal\Delta }
\newcommand{\hbLam}{\hat{\utwi{\mathnormal\Lambda}}}
\newcommand{\hbC}{\hat{\utwi{C}}}
\newcommand{\hbw}{\hat{\utwi{w}}}
\newcommand{\hbm}{\hat{\utwi{m}}}

\newcommand{\tK}{\tilde{K}}
\newcommand{\brK}{\bar{K}}
\newcommand{\brA}{\bar{A}}
\newcommand{\tbd}{\tilde{\bd}}
\newcommand{\tbm}{\tilde{\bm}}
\newcommand{\tbI}{\tilde{\bI}}
\newcommand{\bbI}{\bar{\bI}}
\newcommand{\tbone}{\tilde{\bf 1}}
\newcommand{\bbone}{\bar{\bf 1}}
\newcommand{\tbg}{\tilde{\bg}}
\newcommand{\tbS}{\tilde{\bS}}
\newcommand{\tbA}{\tilde{\bA}}
\newcommand{\tbE}{\tilde{\bE}}
\newcommand{\tbR}{\tilde{\bR}}
\newcommand{\tbM}{\tilde{\bM}}
\newcommand{\bbD}{\bar{\bD}}
\newcommand{\bbC}{\bar{\bC}}
\newcommand{\tbC}{\tilde{\bC}}
\newcommand{\tbD}{\tilde{\bD}}
\newcommand{\bbS}{\bar{\bS}}
\newcommand{\bbT}{\bar{\bT}}
\newcommand{\bbW}{\bar{\bW}}
\newcommand{\bbA}{\bar{\bA}}
\newcommand{\bbE}{\bar{\bE}}
\newcommand{\bbs}{\bar{\bs}}
\newcommand{\bbP}{\bar{\bP}}
\newcommand{\bbR}{\bar{\bR}}
\newcommand{\bbU}{\bar{\bU}}
\newcommand{\tbU}{\tilde{\bU}}
\newcommand{\tbee}{\tilde{\bee}}
\newcommand{\tbP}{\tilde{\bP}}
\newcommand{\bbu}{\bar{\bu}}
\newcommand{\tbu}{\tilde{\bu}}
\newcommand{\tbe}{\tilde{\bee}}
\newcommand{\bbLam}{\bar{\bLam}}
\newcommand{\tbLam}{\tilde{\bLam}}
\newcommand{\bbPsi}{\bar{\bPsi}}
\newcommand{\tbPsi}{\tilde{\bPsi}}
\newcommand{\hbbU}{\hat{\bbU}}
\newcommand{\hbbLam}{\hat{\bbLam}}
\newcommand{\blam}{\bar{\lambda}}
\newcommand{\tlam}{\tilde{\lambda}}

\newcommand{\wun}{\underline{w}}
\newcommand{\sun}{\underline{s}}

